SCOTCH: An Efficient Secure Computation Framework for Secure Aggregation

Federated learning enables multiple data owners to jointly train a machine learning model without revealing their private datasets. However, a malicious aggregation server might use the model parameters to derive sensitive information about the training dataset used. To address such leakage, differential privacy and cryptographic techniques have been investigated in prior work, but these often result in large communication overheads or impact model performance. To mitigate this centralization of power, we propose SCOTCH, a decentralized m-party secure-computation framework for federated aggregation that deploys MPC primitives, such as secret sharing. Our protocol is simple, efficient, and provides strict privacy guarantees against curious aggregators or colluding data-owners with minimal communication overheads compared to other existing state-of-the-art privacy-preserving federated learning frameworks. We evaluate our framework by performing extensive experiments on multiple datasets with promising results. SCOTCH can train the standard MLP NN with the training dataset split amongst 3 participating users and 3 aggregating servers with 96.57% accuracy on MNIST, and 98.40% accuracy on the Extended MNIST (digits) dataset, while providing various optimizations.

==> ppai-appen.tex <==
\section{Appendix}\label{sec:appen}


\subsection{Related Work}\label{subsec:rlwork}

The existing privacy-preserving machine learning (PPML) works focus exclusively on training (generalized) linear models. They rely on \textit{centralized} solutions where the learning task is securely outsourced to a server, notably using homomorphic encryption (HE) techniques. As such, these works do not solve the problem of privacy-preserving distributed ML, where multiple parties collaboratively train an ML model on their data. To address the latter, several works propose multi-party computation (MPC)~\cite{yao1982protocols,lindell2020secure} solutions where several tasks, such as clustering and regression, are distributed among 2, 3, or 4 servers~\cite{mohassel2017secureml,wagh2019securenn,blaze,ramachandran2021s++,wagh2021falcon,riazi2018chameleon,demmler2015aby,payman2018aby3}. Although such approaches, however, limit the number of parties among which the trust is split, often assume an honest majority among the computing servers, and require parties to communicate (i.e., secret share) their data outside their premises. This might not be acceptable due to the privacy and confidentiality requirements and the strict data protection regulations. 

A recently proposed alternative for privacy-preserving training -- without data outsourcing -- is \textit{federated learning} (FL)~\cite{mcmahan2016communication}. FL has emerged as a promising approach to collaboratively train a model by exchanging model parameters with a central aggregator, instead of the actual training data. However, parameter exchange may still leak a significant amount of private data. Several approaches have been proposed to overcome this leakage problem based on differential privacy (DP)~\cite{shokri2015privacy,papernot2018scalable}, MPC~\cite{bonawitz2017practical,ryffel2018generic}, HE~\cite{truex2019hybrid}, Trusted Execution Environment~\cite{mondal2021poster,mondal2021flatee}, etc. Furthermore, in those settings, the aggregator is a central player, which also potentially represents a single point of failure~\cite{kairouz2021advances} and due to the extensive use of cryptographic operations, these frameworks remain too slow for practical use. Finally, other works combine MPC with DP techniques to achieve better privacy guarantees~\cite{truex2019hybrid,xu2019hybridalpha,pettai2015combining}. While DP-based learning aims to mitigate inference attacks, it significantly degrades model utility, as training accurate models requires high privacy budgets~\cite{jayaraman2019evaluating}. Therefore, a \textit{practical} distributed privacy-preserving federated learning approach requires strong cryptographic protection of the intermediate model updates during the model aggregation and the final model weights. 
% In this work, we propose \textsc{Scotch}, a \textit{practical} framework that enables the secure aggregation in a distributed setting and provides end-to-end protection of the parties’ training data, intermediate model weights, and the final resulting model.


\subsection{Dataset and Model configuration}\label{subsec:datamodelconfig}

\subsubsection*{MNIST~\cite{mnist}}
The MNIST~\cite{mnist} dataset comprises 60,000 handwritten digit character images, along with 10,000 testing images. The data is pre-processed by resizing each image, and one-hot encoding the labels. Each client uses a three-layer Multi-layered Perceptron to train on their local datasets. The architecture of the MLP is outlined in Figure~\ref{fig:mlp_arch}.


\subsubsection*{EMNIST}
The Extended MNIST (digits)~\cite{emnist} dataset contains 240,000 handwritten digit character images and 40,000 images for training and testing purposes respectively. The data is preprocessed by resizing each image, and one-hot encoding the labels. We use the same MLP architecture as used in MNIST, to train each local model.

\subsubsection*{FMNIST}
Fashion-MNIST~\cite{fmnist} is a dataset of Zalando's article images that contains 60,000 training images and 10,000 testing images. The data is pre-processed by resizing each image, and one-hot encoding the labels.


% \subsubsection*{Machine Learning Model}

\begin{figure}[ht]
\centering
\includegraphics[width=0.35\textwidth]{figure/MLP_arch.png}
\caption{Multilayer Perceptron (MLP) architecture used across different experiments in \textsc{Scotch}.}
\label{fig:mlp_arch}
\end{figure}




\subsection{Impact of Precision Length}

Most protocols in secure multiparty computation operate in integer rings. However, one needs to deal with decimal numbers while tackling computations in machine learning algorithms. 
To mitigate this, we use a mapping between fixed-point decimals and the integer ring (as used by state-of-the-art MPC frameworks such as SecureML~\cite{mohassel2017secureml}). The integer part of the decimal number is represented by $l_w$ bits and the fractional part by $l_f$. 
To evaluate the effects of precision on our training and testing accuracy, we replicate the precision settings used in SecureML~\cite{mohassel2017secureml} for logistic and linear regression. 
Comparing our tests with SecureML helps us to understand the effects of precision-length while training different machine learning models.
Even though SecureML's experiments were restricted to 13--16 bits, they used  much simpler models such as logistic regression and  with a simpler dataset -- (1000 to 1M samples of the MNIST dataset), and objective -- Binary Classification. 
Through our experiments we observe that multi-class classification via Multi-layer Perceptrons on much smaller dataset 70\% of 60,000 MNIST images performs better if we increase the precision (refer to Table~\ref{table:Centralized}). One might notice how much of a difference does precision make on gradient updates while performing gradient descent using Neural Networks. This difference plays a role in our experiments as well.





\subsection{Performance Accuracy Graph}

\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{figure/SCOTCH_2.png}
\caption{\scriptsize \textsc{Scotch}: Clients vs Performance accuracy on multiple datasets -- MNIST, EMNIST, and FMNIST (3-server setting).}
\label{fig:SCOTCH_plot_acc}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{figure/SCOTCH_(MNIST).png}
\caption{\scriptsize \textsc{Scotch}: Clients vs Performance accuracy on multiple precision settings (16-bits, 32-bits) on MNIST (3-server setting).}
\label{fig:SCOTCH_plot_acc_pre}
\end{figure}






% To overcome this single point of failure, several number of approaches~\cite{bhattacharya,chen,shayan} tries to eliminate the centralized dependence in a learning framework using blockchain technologies and differential privacy (DP). However, due to the extensive use of cryptographic operations, these frameworks remain too slow for practical use. Furthermore, DP decrease the utility of the data and the resulting trained model, and training robust and accurate models requires high privacy budgets, and as such, the level of privacy achieved in practice remains unclear. Therefore, a \textit{practical} distributed privacy-preserving federated learning approach requires strong cryptographic protection of the intermediate model updates during the model aggregation, as well as of the final model weights.

==> secana.tex <==
\section{Privacy Guarantees}\label{sec:secpriv}
\textsc{Scotch} achieves data privacy guarantees under a semi-honest adversary model with any subset of colluding aggregators. \textsc{Scotch}'s infrastructure is designed using multi-input \textit{secret sharing}-based MPC protocol to calculate the federated average of model gradients shared by participating clients. Private training data is not sent -- participating entities get split ``shares'' of model gradients, or the generated averaged model, neither of which can be used to reconstruct sensitive information about the training dataset used. The security of these shares is guaranteed by standard MPC theorems~\cite{goldreich1998secure}, and since the actual computations performed within the MPC setup (which can perform arbitrary computations and is agnostic in that sense). % only output a final model which has standard DP guarantees, no intermediate information is revealed.
